Show Me the Money: Dynamic Recommendations for Revenue Maximization

Recommender Systems (RS) play a vital role in applications such as e-commerce and on-demand content streaming. Research on RS has mainly focused on the customer perspective, i.e., accurate prediction of user preferences and maximization of user utilities. As a result, most existing techniques are not explicitly built for revenue maximization, the primary business goal of enterprises. In this work, we explore and exploit a novel connection between RS and the profitability of a business. As recommendations can be seen as an information channel between a business and its customers, it is interesting and important to investigate how to make strategic dynamic recommendations leading to maximum possible revenue. To this end, we propose a novel \model that takes into account a variety of factors including prices, valuations, saturation effects, and competition amongst products. Under this model, we study the problem of finding revenue-maximizing recommendation strategies over a finite time horizon. We show that this problem is NP-hard, but approximation guarantees can be obtained for a slightly relaxed version, by establishing an elegant connection to matroid theory. Given the prohibitively high complexity of the approximation algorithm, we also design intelligent heuristics for the original problem. Finally, we conduct extensive experiments on two real and synthetic datasets and demonstrate the efficiency, scalability, and effectiveness our algorithms, and that they significantly outperform several intuitive baselines.

==> static.tex <==

\subsection{A Simple Static Model}  \label{sec:static} 
 
%\note[Wei]{This subsection has significant overlap with the second last paragraph of Related Work.Should we consider merge them?} 
%\note[Laks]{Of course. On the one hand, I'd like to suggest that we drop this section, 'cos it seems it says nothing that wasn't said earlier. OTOH, we probably want to hav a ``static'' section, however brief. I will leave it to you to shrink this section drastically, retainng just the core.} 

For completeness, we briefly discuss a static model producing one-shot recommendations.
Instead of a time horizon, merely a single snapshot is considered.
Suppose we know the adoption probability for each user-item pair $(u,i)$, denoted $\ap(u,i)$, and the price of item $i$ at the current time, then  $\ap(u,i) \price(i)$ is the expected revenue generated by recommending $i$ to $u$.
We can then construct a weighted bipartite graph $G = (U\cup I, E)$ with users $U$ and items $I$ as nodes such that for a pair $(u,i) \in U\times I$, the edge weight $w(u,i) = \ap(u,i) \price(i)$.
The edge-set $E\subseteq U\times I$ is simply all $(u,i)$ pairs with $\ap(u,i) > 0$.

Given $G$, $k$ and $q_i$ for all $i$, making recommendations to maximize total expected revenue subject to both display and capacity constraints amounts to finding a \emph{maximum-weight generalized matching}, where an item-node can be matched at most $q_i$ user-nodes and a user-nodes may be match to at most $k$ item-nodes.
As mentioned in Section \ref{sec:related}, this is a special case of a classical graph theoretic problem, \emph{maximum weight degree-constrained subgraphs}, which can be solved optimally in $O( D(|E| + |U\cup I|\log|U\cup I|) )$ time due to Gabow and Tarjan \cite{gabow83, gabow89}.
Here $D$ is the total degree constraints and thus is $k|U| + \sum_{i\in I} q_i$ in our case.

However, their algorithms and also the distributed solution framework by Morales et al. \cite{gianmarco11} and Manshadi et al. \cite{manshadi13} do not deal with the many intricacies involved in the dynamic recommendation strategies.
This is the subject of the remaining subsections.
%Here, the weight of a (generalized) matching is the sum of its edge weights. The item display constraint of at most $k$ recommendations per user can be enforced by saying that in the matching each user node should not have a degree greater than $k$. Similarly, item capacity constraint corresponds to each item node having a degree of at most $q_i$, where $q_i$ is the quantity of item $i$.
%Thus, finding a recommendation strategy to maximize expected revenue under these conditions amounts to finding a \emph{maximum weight degree-constrained subgraph} of the given bipartite graph, which can be solved optimally in polynomial time~\cite{gabow83, gabow89}. 
%\note[Laks]{Cite the authors.} 
%\note[Laks]{State the complexity of their proposed algorithms.} 

\eat{
The recent works by Morales et al. \cite{gianmarco11} and Manshadi et al. \cite{manshadi13} provide efficient distributed framework for this type of problems.
While they are certainly applicable to this static model, as we explained in Sections \ref{sec:intro} and \ref{sec:related}, they do not deal with the many intricacies involved in the dynamic recommendation strategies.
This is the subject of the remaining subsections. 
}


%%%%%%%%%%%%% %%%%%%%%%%%%% %%%%%%%%%%%%% 
%%%%%%%%%%%%% %%%%%%%%%%%%% %%%%%%%%%%%%% 
%%%%%%%%%%%%% BIG EAT  %%%%%%%%%%%%% 
\eat{ 
The corresponding revenue maximization problem can be naturally modeled as a generalized matching problem.
Throughout the paper we use $U$ to denote the set of users and $I$ to denote the set of items.
More specifically, for each user $u\in U$ and each item $i\in I$, a weight $w_{ui}$ is given or learned to represent the revenue the seller expects to make if $i$ is recommended to $u$.
The weight $w_{ui}$ is a highly abstract value that depends on factors such as the price of the item and the likelihood that the user will like the item (and thus make a purchase), etc.

If each user gets to see one item and, vice versa, each item is suggested to no more than one user, at a time, then we are faced with a \emph{maximum weight bipartite matching problem}, which can be solved in polynomial time by the augmenting path algorithm using a shortest path search procedure such as Dijkstra's algorithm and Bellman-Ford algorithm~\cite{algbook}.

More generally, as a common practice, users usually receive a list of up to $k$ recommendations ({\em cf}.\ Amazon and Netflix), where $k$ is determined by the system due to reasons like user-interface design and users' annoyance limit (that is, nobody wishes to see an endless list of recommendations).
In addition, each item $i\in I$ have a certain inventory level (due to supply and demand, shelf life, storage costs, etc), and thus in a short period of time, we may only be able to recommend it to a limited number of users. %, where $q_i$ more or less reflects the inventory level of $i$.
For example, the iPhone 5S in gold was sold out shortly after its release by Apple Inc. on September 20, 2013.
As a retailer, it is not wise to recommend products with tight supply.
It can potentially upset interested buyers since there is a chance for out of stock.
Moreover, there is an obvious opportunity cost of recommending a product that can go out of stock quickly, which is the possible revenue that can be generated by another product that could have been recommended to the user.

Given the aforementioned cardinality constraints on both users and items, the problem becomes to recommend each user $u\in U$ up to $k$ items, such that the expected revenue (total weight) is maximized and no item $i$ is recommended to over $q_i$ users, where $q_i$ is set by the retailer strategically based on $i$'s inventory level.

This more general problem can be viewed as an instance of \emph{maximum weight degree-constrained subgraph problem}, where users in $U$ and items in $I$ are nodes in a graph $G$, and there is an edge between two nodes $u$ and $i$ if $w_{ui}$ is non-zero.
The task is to find a subgraph of $G$ constructed like above, such that in this subgraph, first, the cardinality constraints are respected -- the degree of a user node $u$ is at most $k$ and the degree of an item node $i$ is at most $q_i$ -- and second, the sum of the weights in this subgraph is the largest amongst all subgraphs of $G$ respecting the degree constraints ($k$ and $q_i$).
The maximum weight degree-constrained subgraph problem was studied extensively by Gabow and Tarjan \cite{gabow83, gabow89}, in which polynomial-time algorithms were proposed.

\note[Wei]{Mention the vldb matching papers (german and y! barcelona?) and say they are only static and not interesting}

To summarize, for static one-shot recommendations, revenue maximization can be formulated as generalized matching problems and solved optimally in polynomial time.
However, this setting is in highly coarse granularity as the intricacy of user-item interactions are entirely encapsulated into the weights $w_{ui}$'s.
%Next, we extend our problem setting beyond a single snapshot and consider various factors that affect recommendation-based revenue.
} 
%%%%%%%%%%%%%%%%% END BIG EAT 

